Elliptic boundary-value problems in H\"ormander spaces

We investigate general elliptic boundary-value problems in H\"ormander inner product spaces that form the extended Sobolev scale. The latter consists of all Hilbert spaces that are interpolation spaces with respect to the Sobolev Hilbert scale. We prove that the operator corresponding to an arbitrary elliptic problem is Fredholm in appropriate couples of the H\"ormander spaces and induces a collection of isomorphisms on the extended Sobolev scale. We obtain a local a priory estimate for generalized solutions to this problem and prove a theorem on their local regularity in the H\"ormander spaces. We find new sufficient conditions under which generalized derivatives (of a given order) of the solutions are continuous.

==> jinfo.tex <==
\jvolume{22}
\jyear{2016}
\jnumber{4}

